Mastering Diverse Domains through World Models

Developing a general algorithm that learns to solve tasks across a wide range of applications has been a fundamental challenge in artificial intelligence. Although current reinforcement learning algorithms can be readily applied to tasks similar to what they have been developed for, configuring them for new application domains requires significant human expertise and experimentation. We present DreamerV3, a general algorithm that outperforms specialized methods across over 150 diverse tasks, with a single configuration. Dreamer learns a model of the environment and improves its behavior by imagining future scenarios. Robustness techniques based on normalization, balancing, and transformations enable stable learning across domains. Applied out of the box, Dreamer is the first algorithm to collect diamonds in Minecraft from scratch without human data or curricula. This achievement has been posed as a significant challenge in artificial intelligence that requires exploring farsighted strategies from pixels and sparse rewards in an open world. Our work allows solving challenging control problems without extensive experimentation, making reinforcement learning broadly applicable.

==> Makefile <==
engine = "pdflatex -interaction=nonstopmode --shell-escape %O %S"
refs = main.bib
sources = main.tex $(shell find . -type f -name '*.tex')

main.pdf: $(sources)
	@latexmk -pdf -pdflatex=${engine} -output-directory='output' -bibtex $<

watch:
	make; \
	(zathura output/main.pdf &); \
	while true; do \
		inotifywait -e modify -q $(sources); \
		make; \
	done
	# @while inotifywait -e modify $(refs) $(sources); do make; done

spell:
	@hunspell -l -t -d en_US -i utf-8 $(sources) \
		| sort \
		| uniq --ignore-case \
		| grep -vxFf dictionary.txt

clean:
	@latexmk -C
	rm main.bbl || true
	rm -rf output/*

pack:
	cp output/main.bbl main.bbl
	rm ../dreamerv3.zip || true
	zip -r ../dreamerv3.zip . -x '*.git*' -x 'output/*'
	# rm ../dreamerv3.tar || true
	# tar -czvf ../dreamerv3.tar --exclude .git --exclude output --exclude .gitignore  .

.PHONY: watch spell clean


==> figures/bars/figure.tex <==
\begin{figure}[t!]
\centering
\vspace*{-2ex}%
\includegraphics[width=\linewidth]{bars/bars}
\vspace*{-3ex}%
\caption{Benchmark scores. Using fixed hyperparameters across all domains, Dreamer outperforms tuned expert algorithms across a wide range of benchmarks and data budgets. Dreamer also substantially outperforms a high-quality implementation of the widely applicable PPO algorithm.}
\label{fig:bars}
\end{figure}

==> figures/minecraft/figure.tex <==
\begin{figure}[t]
\centering
\vspace*{-4ex}%
\includegraphics[width=\linewidth]{figures/minecraft/minecraft}%
\caption{Performance on the Minecraft Diamond challenge.
\textbf{a}, Applied out of the box, Dreamer is the first algorithm to accomplish all 12 milestones leading up to the diamond, from sparse rewards without human data or curricula.
\textbf{b}, Fraction of trained agents that discover each of the three latest items in the diamond task. Although previous algorithms progress up to the iron pickaxe, Dreamer is the only compared algorithm that manages to discover a diamond, and does so reliably.
The shaded areas indicate one standard deviation.
}
\label{fig:minecraft}
\end{figure}

